Probabilistic Dataset Reconstruction from Interpretable Models

Interpretability is often pointed out as a key requirement for trustworthy machine learning. However, learning and releasing models that are inherently interpretable leaks information regarding the underlying training data. As such disclosure may directly conflict with privacy, a precise quantification of the privacy impact of such breach is a fundamental problem. For instance, previous work have shown that the structure of a decision tree can be leveraged to build a probabilistic reconstruction of its training dataset, with the uncertainty of the reconstruction being a relevant metric for the information leak. In this paper, we propose of a novel framework generalizing these probabilistic reconstructions in the sense that it can handle other forms of interpretable models and more generic types of knowledge. In addition, we demonstrate that under realistic assumptions regarding the interpretable models' structure, the uncertainty of the reconstruction can be computed efficiently. Finally, we illustrate the applicability of our approach on both decision trees and rule lists, by comparing the theoretical information leak associated to either exact or heuristic learning algorithms. Our results suggest that optimal interpretable models are often more compact and leak less information regarding their training data than greedily-built ones, for a given accuracy level.

==> rule_list_example_gen_old.tex <==
\input{example_rule_list}

The algorithm reconstructing a probabilistic version of a rule list $\rulelist$'s training set from $\rulelist$ itself simply follows the path of each example. 
For an example classified by the $\ruleindex$th rule, it reduces the domains of the attributes involved in the  $\ruleindex$th rule accordingly. It also eliminates all attributes' conjunctions contradicting the fact that the example did not match the previous rules within $\rulelist$.
For instance, the following knowledge can be extracted from Rule List~\ref{rl:example}:\begin{itemize}
    \item The \textbf{first rule} indicates that for $1644 + 802 = 2446$ examples, we can reduce the domains of the two Boolean attributes \texttt{Age>=30} and \texttt{Prior-Crimes>5}.
    \item Using the \textbf{second rule}, we can filter the domains of the two Boolean attributes \texttt{Prior-Crimes=0} and \texttt{Age=18-22} for $345+160=505$ examples. \emph{Furthermore, we know that the conjunction \texttt{Age>=30 and Prior-Crimes>5} is not possible for these examples.} 
    \item Finally, the \textbf{default rule} states that for $965+1855=2820$ examples, \emph{the conjunctions \texttt{Age>=30 and Prior-Crimes>5} and \texttt{Prior-Crimes=0 and Age=18-22} are not possible}.
\end{itemize} 
    
In this example, part of the model's knowledge directly reduces the individual domains of some attributes for the examples concerned.
As such, the information it brings will successfully be quantified by $\oldmetric$ and encoded in a probabilistic dataset.
However, the \emph{knowledge specified in italic} does not reduce any attribute's domain \emph{individually}. 
While such knowledge brings information for reconstruction, this cannot be quantified using $\oldmetric$ nor represented using a probabilistic dataset as formalized in Definition~\ref{def:probabilistic_datasets}.

==> toy_example_dataset_dumb.tex <==
\begin{table}[]
\begin{tabular}{c|c|c|c|c|}
\cline{2-5}
                                     & $\singleattribute_1$              & $\singleattribute_2$ & $\singleattribute_3$ & Label           \\ \hline
\multicolumn{1}{|c|}{$\anexample_1$} & $ \in \{10, 11, 12, 13, 14, 15\}$ & $ \in \{0, 1\}$      & $ \in \{1, 2, 3\}$   & $ \in \{0, 1\}$ \\ \hline
\multicolumn{1}{|c|}{$\anexample_2$} & $ \in \{10, 11, 12, 13, 14, 15\}$ & $ \in \{0, 1\}$      & $ \in \{1, 2, 3\}$   & $ \in \{0, 1\}$ \\ \hline
\multicolumn{1}{|c|}{$\anexample_3$} & $ \in \{10, 11, 12, 13, 14, 15\}$ & $ \in \{0, 1\}$      & $ \in \{1, 2, 3\}$   & $ \in \{0, 1\}$ \\ \hline
\multicolumn{1}{|c|}{$\anexample_4$} & $ \in \{10, 11, 12, 13, 14, 15\}$ & $ \in \{0, 1\}$      & $ \in \{1, 2, 3\}$   & $ \in \{0, 1\}$ \\ \hline
\end{tabular}
\end{table}

==> toy_example_dataset_orig.tex <==
\begin{table}[]
\begin{tabular}{c|c|c|c|c|}
\cline{2-5}
                                     & $\singleattribute_1$ & $\singleattribute_2$ & $\singleattribute_3$ & Label \\ \hline
\multicolumn{1}{|c|}{$\anexample_1$} & 12                   & 0                    & 3                    & 0     \\ \hline
\multicolumn{1}{|c|}{$\anexample_2$} & 14                   & 1                    & 2                    & 0     \\ \hline
\multicolumn{1}{|c|}{$\anexample_3$} & 11                   & 1                    & 2                    & 1     \\ \hline
\multicolumn{1}{|c|}{$\anexample_4$} & 14                   & 0                    & 1                    & 1     \\ \hline
\end{tabular}
\end{table}

==> toy_example_dataset_rec.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|c|c|}
\hline
               & $\singleattribute_1$              & $\singleattribute_2$ & $\singleattribute_3$ & Label \\ \hline
$\anexample_1$ & $ \in \{12, 13, 14, 15\}$         & $ \in \{0, 1\}$      & $ \in \{2, 3\}$      & 0     \\ \hline
$\anexample_2$ & $ \in \{12, 13, 14, 15\}$         & $ \in \{0, 1\}$      & $ \in \{2, 3\}$      & 0     \\ \hline
$\anexample_3$ & $ \in \{10, 11\}$                 & $ \in \{0, 1\}$      & $ \in \{2, 3\}$      & 1     \\ \hline
$\anexample_4$ & $ \in \{10, 11, 12, 13, 14, 15\}$ & $ \in \{0, 1\}$      & $ \in \{1\}$         & 1     \\ \hline
\end{tabular}
\end{table}
